Multi-HMR: Multi-Person Whole-Body Human Mesh Recovery in a Single Shot

We present Multi-HMR, a strong sigle-shot model for multi-person 3D human mesh recovery from a single RGB image. Predictions encompass the whole body, i.e., including hands and facial expressions, using the SMPL-X parametric model and 3D location in the camera coordinate system. Our model detects people by predicting coarse 2D heatmaps of person locations, using features produced by a standard Vision Transformer (ViT) backbone. It then predicts their whole-body pose, shape and 3D location using a new cross-attention module called the Human Prediction Head (HPH), with one query attending to the entire set of features for each detected person. As direct prediction of fine-grained hands and facial poses in a single shot, i.e., without relying on explicit crops around body parts, is hard to learn from existing data, we introduce CUFFS, the Close-Up Frames of Full-Body Subjects dataset, containing humans close to the camera with diverse hand poses. We show that incorporating it into the training data further enhances predictions, particularly for hands. Multi-HMR also optionally accounts for camera intrinsics, if available, by encoding camera ray directions for each image token. This simple design achieves strong performance on whole-body and body-only benchmarks simultaneously: a ViT-S backbone on $448{\times}448$ images already yields a fast and competitive model, while larger models and higher resolutions obtain state-of-the-art results.

==> abbrev.tex <==
% ---------------------------------------------------------------
%
% Formatting Package for ECCV Submissions
% 
% initially created for ECCV 2024
% by Stefan Roth
%
% based on previous ECCV templates:
%   updated April 2002 by Antje Endemann
%   Based on CVPR 07 and LNCS, with modifications by DAF, AZ and elle, 2008 and AA, 2010, and CC, 2011; TT, 2014; AAS, 2016; AAS, 2020; TH, 2022
%
% and the CVPR templates:
%   https://github.com/cvpr-org/author-kit
%
% No guarantee is given that the format corresponds perfectly to
% LNCS Proceedings, but most features should be ok.
%
% ---------------------------------------------------------------

\NeedsTeXFormat{LaTeX2e}[1999/12/01]
% \ProvidesPackage{eccvabbrv}[Common abbreviations for ECCV]

% Add a period to the end of an abbreviation unless there's one
% already, then \xspace.
\RequirePackage{xspace}
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\emph{e.g}\onedot} 
\def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} 
\def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{cf}\onedot} 
\def\Cf{\emph{Cf}\onedot}
\def\etc{\emph{etc}\onedot} 
\def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} 
\def\dof{d.o.f\onedot}
\def\iid{i.i.d\onedot} 
\def\wolog{w.l.o.g\onedot}
\def\etal{\emph{et al}\onedot}
\makeatother

% Redefine \emph{} to always produce italic text
\makeatletter
\renewcommand{\emph}[1]{{\itshape #1}}
\makeatother

% checkmarks
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
\definecolor{MyGreen}{RGB}{0,128,0}
\definecolor{MyRed}{RGB}{220,20,60}
\newcommand*{\boldcheckmark}{%
  \textpdfrender{
    TextRenderingMode=FillStroke,
    LineWidth=1.2pt,
  }{\checkmark}
}
\newcommand{\greencheck}{{\color{MyGreen}\boldcheckmark}}
\newcommand{\redxmark}{{\color{MyRed}\xmark}}%
\newcommand{\greencmark}{{\color{MyGreen}\cmark}}

% weird stuff for the font of the tikz figures
\makeatletter
\usepackage{trimspaces}
\def\trimspace#1{\trim@spaces@in{#1}}
\newcommand\HUGE{\@setfontsize\Huge{31}{39}}
\makeatother

%%%%%%%%%%%%
\newlength\savewidth\newcommand\shline{\noalign{\global\savewidth\arrayrulewidth
\global\arrayrulewidth 1pt}\hline\noalign{\global\arrayrulewidth\savewidth}}
\newcommand{\tablestyle}[2]{\setlength{\tabcolsep}{#1}\renewcommand{\arraystretch}{#2}\centering\footnotesize}
\renewcommand{\paragraph}[1]{\vspace{1.25mm}\noindent\textbf{#1}}
\newcommand\blfootnote[1]{\begingroup\renewcommand\thefootnote{}\footnote{#1}\addtocounter{footnote}{-1}\endgroup}

\newcolumntype{x}[1]{>{\centering\arraybackslash}p{#1pt}}
\newcolumntype{y}[1]{>{\raggedright\arraybackslash}p{#1pt}}
\newcolumntype{z}[1]{>{\raggedleft\arraybackslash}p{#1pt}}

\newcommand{\app}{\raise.17ex\hbox{$\scriptstyle\sim$}}
\newcommand{\mypm}[1]{\color{gray}{\tiny{$\pm$#1}}}
\newcommand{\x}{{\times}}
\definecolor{deemph}{gray}{0.6}
\newcommand{\gc}[1]{\textcolor{deemph}{#1}}
\definecolor{baselinecolor}{gray}{.9}
\newcommand{\baseline}[1]{\cellcolor{baselinecolor}{#1}}
\newcommand{\authorskip}{\hspace{2.5mm}}

% General use commands
\newcommand{\myparagraph}[1]{\vspace{0.05cm} \noindent \textbf{#1.}}
\newcommand{\mydataset}[1]{\noindent \textbf{#1} }
\newcommand{\ours}{Multi-HMR\xspace}
\newcommand{\Ours}{Multi-HMR\xspace}
\newcommand{\onestage}[0]{single-shot\xspace}
\newcommand{\Onestage}[0]{Single-shot\xspace}
\newcommand{\dataset}{CUFFS\xspace}
\newcommand{\datasetname}{Close-Up Frames of Full-body Subjects\xspace}

\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\orange}[1]{\textcolor{orange}{#1}} 
\newcommand{\hlcell}[0]{\cellcolor{gray!22}} % For higlighting in tables

\hyphenation{sim-pli-ci-ty}

% colors for table
\definecolor{tabzeroth}{rgb}{1, 0.5, 0.5}
\definecolor{tabfirst}{rgb}{1, 0.7, 0.7} %# red
\definecolor{tabsecond}{rgb}{1, 0.85, 0.7}% # orange
\definecolor{tabthird}{rgb}{1, 1, 0.7} %# yellow

% input
\input{math_commands.tex}
\input{pgfstyles.tex}

\graphicspath{{figs/}}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%



% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rvdelta{{\mathbf{\delta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{d}} %\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{f}} %\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\eta}} %\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\valpha{{\bm{\alpha}}}
\def\vbeta{{\bm{\beta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> pgfstyles.tex <==
\newcommand{\convexhullmarkersize}{2.5pt}
\newcommand{\convexhullmarkeropacity}{0.75}

\newcommand{\multicropc}{Gray}
\newcommand{\lonec}{MidnightBlue}
\newcommand{\loneorthc}{SkyBlue}
\newcommand{\loneocmc}{Blue}
\newcommand{\ltwoc}{Magenta}
\newcommand{\ltwoorthc}{Lavender}
\newcommand{\ltwoocmc}{RedViolet}
\newcommand{\lthreec}{Green}
\newcommand{\lthreeorthc}{YellowGreen}
\newcommand{\lthreeocmc}{OliveGreen}
\newcommand{\ocmc}{Plum}
\newcommand{\ocac}{Brown}

\newcommand{\trexc}{\loneocmc}
\newcommand{\trexsc}{\lthreeocmc}

\newcommand{\base}{Base}
\newcommand{\basemc}{\base+Mc}
\newcommand{\basemcshort}{\,+Mc}
\newcommand{\basepr}{\base+Pr}
\newcommand{\baseprshort}{\,+Pr}
\newcommand{\basemcpr}{\base+Mc+Pr}
\newcommand{\basemcprshort}{\,+Mc+Pr}
\newcommand{\basebs}{\base{} (BS=2K)}
\newcommand{\featureanalysismarkeropacity}{0.75}

\newcommand{\baseprc}{Orange}
\newcommand{\basemcprc}{Brown}
\newcommand{\basemcpronec}{Brown}

\newcommand{\ocmmcpronec}{Blue}
\tikzstyle{ocmmcprone} = [line width=1.5pt, dashed, color=\ocmmcpronec, mark=+]


\newcommand{\basebsc}{Black}
\tikzstyle{basebs} = [line width=1.5pt, color=\basebsc]
\tikzstyle{basemc} = [line width=1.5pt, color=\basemcc]
\tikzstyle{basepr} = [line width=1.5pt, color=\baseprc]
\tikzstyle{basemcprone} = [line width=1.5pt, dashed, color=\basemcpronec, mark=o]



\tikzstyle{arrowmc} = [dashed, opacity=0.5, line width=1pt, color=\multicropc, shorten >= 6pt, shorten <= 6pt, -{Latex[round]}]
\tikzstyle{arrowpr} = [dashed, opacity=0.5, line width=1pt, color=\baseprc, shorten >= 6pt, shorten <= 6pt, -{Latex[round,open]}]



\newcommand{\rsbc}{black}
\newcommand{\lookc}{black}
\newcommand{\supconc}{black}
\newcommand{\dinoc}{black}
\newcommand{\bonec}{OrangeRed}
\newcommand{\btwoc}{Orange}
\newcommand{\mcc}{Purple}

\newcommand{\dinovtwoc}{YellowGreen}
\newcommand{\mupodec}{OrangeRed}

\pgfmathsetmacro{\teasermarkersize}{3}
\pgfmathsetmacro{\stdgrad}{10}


\tikzset{every mark/.append style={solid}}
\pgfplotsset{
	grid=both, width=\linewidth, try min ticks=5,
	legend cell align=left, legend style={fill opacity=0.8},
	ylabel near ticks,
    xlabel near ticks,
    every tick label/.append style={font=\footnotesize},
}

\pgfplotsset{
     rsb/.style={ultra thick, color=\rsbc, mark=x,mark size=\teasermarkersize pt, only marks},
    dino/.style={ultra thick, color=\dinoc, mark=+,mark size=\teasermarkersize pt, only marks},
    dinov2/.style={ultra thick, color=\dinov2c, mark=+,mark size=\teasermarkersize pt, only marks},
    paws/.style={ultra thick, color=\dinoc, mark=Mercedes star flipped,mark size=\teasermarkersize pt, only marks},
    slmlp/.style={thick, color=\lookc, mark=diamond*,mark size=\teasermarkersize pt, only marks, every mark/.append},
    look/.style={thick, color=\lookc, mark=square*,mark size=\teasermarkersize-1 pt, only marks, every mark/.append style={rotate=45}},
    supcon/.style={thick, color=\supconc, mark=pentagon*,mark size=\teasermarkersize pt, only marks},
    mc/.style={thick, color=\mcc, mark=*,mark size=\teasermarkersize-1 pt, only marks},
    bone/.style={thick, color=\bonec, mark=triangle*,mark size=\teasermarkersize pt, only marks},
    btwo/.style={thick, color=\btwoc, mark=triangle*,mark size=\teasermarkersize pt, only marks, every mark/.append style={rotate=-90}}
    
}

\pgfplotsset{
    multicrop/.style={color=\multicropc, mark=*, mark size=\convexhullmarkersize, only marks},
    lone/.style={color=\lonec, mark=*, mark size=\convexhullmarkersize, only marks},
    loneorth/.style={color=\loneorthc, mark=pentagon*, mark size=\convexhullmarkersize, only marks},
    ltwo/.style={color=\ltwoc, mark=*, mark size=\convexhullmarkersize, only marks},
    ltwoorth/.style={color=\ltwoorthc, mark=pentagon*, mark size=\convexhullmarkersize, only marks},
    lthree/.style={color=\lthreec, mark=*, mark size=\convexhullmarkersize, only marks},
    lthreeorth/.style={color=\lthreeorthc, mark=pentagon*, mark size=\convexhullmarkersize, only marks},
    ocm/.style={color=\ocmc, mark=triangle*, mark size=\convexhullmarkersize+1, only marks},
    oca/.style={color=\ocac, mark=diamond*, mark size=\convexhullmarkersize+1, only marks},
    ocmlone/.style={color=\loneocmc, mark=triangle*, mark size=\convexhullmarkersize+1, only marks},
    ocmltwo/.style={color=\ltwoocmc, mark=triangle*, mark size=\convexhullmarkersize+1, only marks},
    ocmlthree/.style={color=\lthreeocmc, mark=triangle*, mark size=\convexhullmarkersize+1, only marks},
    trex/.style={color=\trexc, mark=star, mark size=\convexhullmarkersize+1, ultra thick, only marks},
    trexs/.style={color=\trexsc, mark=star, mark size=\convexhullmarkersize+1, ultra thick, only marks},
    base/.style={color=\basec, draw=black, mark=square*, mark size=\convexhullmarkersize, only marks},
    basemc/.style={color=\basemcc, mark=triangle*, mark size=\convexhullmarkersize+1.5, mark options={rotate=180}, only marks},
    basepr/.style={color=\baseprc, mark=triangle*, mark size=\convexhullmarkersize+1.5, only marks},
    basemcpr/.style={color=\basemcprc, mark=square*, mark size=\convexhullmarkersize, mark options={rotate=45}, only marks},
}

\usetikzlibrary{tikzmark}
\pgfplotsset{compat=newest}
\usepgfplotslibrary{fillbetween}
\usepgfplotslibrary{colorbrewer}
\usepgfplotslibrary{colormaps}
\usetikzlibrary{arrows.meta}
\usetikzlibrary{patterns}
\usetikzlibrary{external}

\newcolumntype{a}{>{\columncolor[gray]{.9}[.5\tabcolsep]}c}

\newcommand{\yoloOsxc}{Bittersweet}
\tikzstyle{yoloOsx} = [line width=1.5pt, dashed, color=\basemcpronec, mark=o]
\newcommand{\rompc}{Blue}
\tikzstyle{romp} = [line width=1.5pt, dashed, color=\ocmmcpronec, mark=+]

\newcommand{\bbdinovtwosc}{BrickRed}
\tikzstyle{bbdinovtwos} = [line width=1.5pt, color=\bbdinovtwosc, mark=o]
\newcommand{\bbdinovtwosb}{BurntOrange}
\tikzstyle{bbdinovtwob} = [line width=1.5pt, color=\bbdinovtwosb, mark=x]
\newcommand{\bbdinovtwolc}{NavyBlue}
\tikzstyle{bbdinovtwol} = [line width=1.5pt, color=\bbdinovtwolc, mark=+]
\tikzstyle{sotastyle} = [line width=1.5pt, dashed, color=ForestGreen, mark=x, mark size=3pt]

\tikzstyle{dinov2} = [line width=1.5pt, color=\baseprc, mark=o]
\tikzstyle{dino} = [line width=1.5pt, color=\basemcprc, mark=o]
\tikzstyle{vitpose} = [line width=1.5pt, color=\ocmmcpronec, mark=o]

\tikzstyle{sotaline} = [line width=0.8pt, color=ForestGreen, dashed, mark=x,mark size=3pt]

\newcommand{\spideronec}{}
\newcommand{\spidertwoc}{Bittersweet}
\newcommand{\spiderthreec}{NavyBlue}
\newcommand{\spiderfourc}{OrangeRed}

\newcommand{\mubasec}{Bittersweet}
\newcommand{\mubaserayc}{NavyBlue}
\newcommand{\mubaserayfnc}{OrangeRed}
\newcommand{\mubasevthreedc}{Emerald}
\newcommand{\mubasevtwodc}{Black}

\newcommand{\mucrossc}{Emerald}
